TRUST: An LLM-Based Dialogue System for Trauma Understanding and Structured Assessments

Objectives: While Large Language Models (LLMs) have been widely used to assist clinicians and support patients, no existing work has explored dialogue systems for standard diagnostic interviews and assessments. This study aims to bridge the gap in mental healthcare accessibility by developing an LLM-powered dialogue system that replicates clinician behavior. Materials and Methods: We introduce TRUST, a framework of cooperative LLM modules capable of conducting formal diagnostic interviews and assessments for Post-Traumatic Stress Disorder (PTSD). To guide the generation of appropriate clinical responses, we propose a Dialogue Acts schema specifically designed for clinical interviews. Additionally, we develop a patient simulation approach based on real-life interview transcripts to replace time-consuming and costly manual testing by clinicians. Results: A comprehensive set of evaluation metrics is designed to assess the dialogue system from both the agent and patient simulation perspectives. Expert evaluations by conversation and clinical specialists show that TRUST performs comparably to real-life clinical interviews. Discussion: Our system performs at the level of average clinicians, with room for future enhancements in communication styles and response appropriateness. Conclusions: Our TRUST framework shows its potential to facilitate mental healthcare availability.

==> tex/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\paragraph{Dialogue Acts Schema} Dialogue Acts have been employed in modeling
both general conversations \citep{Godfrey1992} and task-oriented interactions \citep{Boyer2010},
yet research on dialogue act schemas in healthcare remains limited.
Existing work primarily addresses specific behaviors in therapy or interviews \citep{Perez-Rosas2016,Guntakandla2018},
with few studies exploring diagnostic contexts.
\citet{Bifis2021} developed a multi-level taxonomy with 30 terminal nodes for telehealth applications,
while \citet{Xu2023} identified seven dialogue acts from medical consultation datasets.
Most relevant to our work, \citet{Farzana2020} created a dialogue act schema for dementia screening interviews.
Our approach uniquely focuses on the clinician side of diagnostic interviews,
providing a guidance for dialogue systems to generate appropriate clinical responses given context,
a distinct contribution to healthcare dialogue modeling.


\paragraph{Clinical Dialogue System} Since the advent of LLMs,
researchers have explored their applications in medical dialogue systems,
focusing on areas such as clinical reasoning \citep{Tang2024},
mental health counseling \citep{Bao2023},
and medical question answering \citep{Singhal2025}.
However, few studies have addressed dialogue systems for automatic diagnosis.
\citet{Chen2023} proposed KNSE, a knowledge-aware natural language inference (NLI) framework
for dialogue symptom status recognition in medical conversations.
\citet{Chen2023a} investigated the feasibility of using ChatGPT to simulate both doctors and patients,
employing prompt engineering guided by psychiatrists.
Despite these advancements, there remains a research gap in systems capable of
conducting long-time diagnostic interviews for assessments.

\paragraph{LLM-powered Simulation} There is an increasing interest in leveraging LLMs
to simulate various roles for professional training,
particularly in domains such as education \citep{Markel2023} and counseling \citep{Chen2023a}.
\citet{louie-etal-2024-roleplay} introduced Roleplay-doh, an innovative pipeline that
incorporates domain expert feedback to simulate patients and train novice counselors in mental health settings.
Similarly, \citet{Wang2024} developed Patient-$\Psi$,
which employs cognitive modeling to simulate patients for cognitive behavioral therapy (CBT) training.
Our system distinguishes itself by utilizing real-life interview transcripts as the source for patient simulation,
ensuring more authentic and clinically accurate interactions.

